Beyond Gradient and Priors in Privacy Attacks: Leveraging Pooler Layer Inputs of Language Models in Federated Learning

Language models trained via federated learning (FL) demonstrate impressive capabilities in handling complex tasks while protecting user privacy. Recent studies indicate that leveraging gradient information and prior knowledge can potentially reveal training samples within FL setting. However, these investigations have overlooked the potential privacy risks tied to the intrinsic architecture of the models. This paper presents a two-stage privacy attack strategy that targets the vulnerabilities in the architecture of contemporary language models, significantly enhancing attack performance by initially recovering certain feature directions as additional supervisory signals. Our comparative experiments demonstrate superior attack performance across various datasets and scenarios, highlighting the privacy leakage risk associated with the increasingly complex architectures of language models. We call for the community to recognize and address these potential privacy risks in designing large language models.

==> src/8-misc/contributions.tex <==

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

==> src/rebuttal/common.tex <==
Dear Reviewers,

We sincerely appreciate your insightful feedback and have comprehensively revised our manuscript to address your concerns. If these modifications address your initial queries, we'd be grateful if you could revise your evaluation accordingly. Below is a summary of the critical modifications we have implemented:

1. **Clarification on Threat and Security Models:**
   - Responding to Reviewers 1dmy and eYy2, we've clarified our threat and security models, as well as the high-level categorization of our method. These clarifications are now included in the introduction (highlighted in red and blue in the second paragraph) and in the related work section (in the last two paragraphs, also highlighted). Furthermore, a systematic discussion of these models is provided in Appendix-A.

2. **Distinction from Previous Studies:**
   - To address concerns from Reviewers 1dmy and tBfV about how our work differs from previous studies, we've made relevant modifications in the sections mentioned above. Additionally, we have included a comparative analysis in Appendix-A, presented in a tabular format.

3. **Discussion on Method Constraints:**
   - For Reviewer tBfV's query about method constraints, we have added detailed discussions and responses in Appendix A-1 and A-2.

4. **Explanation of Two-Layer Neural Network-Based Reconstruction Method:**
   - Addressing queries from Reviewers 1dmy and tBfV regarding the two-layer-neural-network-based reconstruction method, we have provided an in-depth explanation and justification in Appendix C-1.

5. **First Use of Intermediate Feature in Privacy Textual Data Attack:**
   - In response to Reviewers eYy2 and 1dmy, we have elaborated in Appendix C-2 on whether our introduction of the intermediate feature constitutes a first in privacy textual data attack.

6. **Objectivity in Presentation:**
   - Reviewer 1dmy's concern about objectivity has been addressed by highlighting changes in the manuscript, focusing on the sections emphasized by the reviewer.

7. **Clarification of Notations:**
   - To clarify the notation issues raised by Reviewer eYy2, we have made modifications in the relevant sections, indicated by highlighted text.

8. **Rationale Behind Using Cosine Similarity in Optimization:**
   - Lastly, in response to Reviewer 1dmy's question about using cosine similarity in optimization, we have provided a comprehensive explanation at the end of Appendix C-1.

9. **Direct Responses on OpenReview:**

    - For some inquiries that were not explicitly reflected in the revised version of our manuscript, we invite reviewers and readers to view our direct responses on OpenReview. We have provided detailed explanations and justifications there to address these specific queries, ensuring comprehensive coverage of all concerns raised.

We believe these revisions significantly enhance the clarity, rigor, and contribution of our work. We thank you for your constructive feedback, which has been invaluable in improving the quality and impact of our research.


==> src/rebuttal/rebuttal-1.tex <==
Thank you for your constructive feedback. Below are our responses to your main concerns. If these address your initial queries, we'd be grateful if you could revise your evaluation accordingly.

### Question 1: Clarification of Threat Model

We are thankful for the reviewer's astute observation that our discussion has been primarily focused on the optimization perspective without a high-level exploration of our threat model. This approach is indeed a result of deep contemplation.

1. **Classification of Attacks:**
Following previous work, we categorized attacks as Malicious and Eavesdropping (or Honest-but-Curious Server) Attacks, but this oversimplifies the issue. Traditional Malicious Attacks involve altering server states or model architecture, rendering gradient information useless. However, our method, which only modifies the Pooler layer of the model, doesn't affect the original training purpose, thus differing from typical Malicious Attacks.

2. **Wider Pooler Layer:**
The width of Pooler Layer depends on the recovery needs. For a small input portion (X' with d_r << d_in), the required width reduces significantly, as detailed in **Section 4: Flexibility of Recovered Dimension**. With the growth of Large Language Models like GPT-3, which already exceeds the necessary dimensions (12288 for d_r = 50), this width requirement becomes less vital. Moreover, our attack focuses on wide models, aligning with previous studies [Geiping et al.2020, Fowl et al.2022], revealing more risk in our settings.

3. **Activation Functions Change:**
We've identified risks with activation functions like Silu, lacking purely even or odd higher-order derivatives. Our ongoing research explores activation functions with strictly odd or even derivatives, like tanh or relu. Many previous studies strengthen particular activation functions [Zhu et al. 2019]; we claim our discovery is a contribution instead of a drawback.

4. **Redefining 'Honest-but-Curious':**
Compared to Eavesdropping (Honest-but-Curious) attacks, our method does involve some modifications to the model. `However, we propose that 'honest' should not be narrowly defined as the server's absolute fidelity to clients. Instead, 'honest' should be understood as the server's adherence to its primary role of obtaining effective gradients and minimizing the model's loss function.` By this definition, our approach falls under the Honest-but-Curious category.

5. **Clarifying Our Method's Positioning:**
In summary, our method cannot be classified as a Malicious or Eavesdropping Attack unless we redefine the Honest-but-Curious category. Our method, compared to Malicious Attacks, is more difficult to detect and does not violate the fundamental objective of federated learning. In contrast to Eavesdropping Attacks, our approach achieves more effective outcomes. Therefore, we mainly discuss our method from the perspective of optimization.

6. **Elaborating on the Threat Model:**
    - We do not fine-tune the model's word and positional embeddings. The gradients for these embeddings are non-zero for words in the client's training data, enabling easy recovery of client sequences.
    - The server operates under a redefined 'honest but curious' model, aiming to learn maximally from gradients without altering the learning protocol.

7. **Appendix for Enhanced Understanding:**
To aid the reviewer's understanding, we will include a table in the appendix of our revised manuscript. This table will delineate the differences between Malicious Attacks, Eavesdropping Attacks, and Honest-but-Curious Server attacks, with examples from previous work (LAMP, Wang et al. 2023).

### Question 2: Novelty Concern

Thank you for your comments on our work's novelty. We want to clarify a few points:
1. **Contribution Clarification:**
    - Our contribution isn't about identifying gradient-based attack issues, which was just an analysis foundation. Our innovation is in our unique approach to protecting textual data privacy using intermediate features.

2. **Differentiation from Prior Work [1]:**
    - We recognize similar use of intermediate features in previous studies [1] on **image data**. However, our work pioneers this concept for **textual data attacks**, facing unique challenges not seen in image data due to differences in data representation and model architectures.
    - Our technique method is totally different from [1]

### Question 3: Tone and Subjectivity
Thank you for pointing out the subjective tone. We will revise this. **The term "revolutionary" was specifically for our new metric on textual data information leakage, not our method (Contribution 4)**.

### Question 4: Optimization Objective
I appreciate your insight on our optimization objective. We aim to recover the directional component of the Pooler layer's input using decomposition, acknowledging challenges in reconstructing its magnitude. Our solution employs cosine similarity loss to address this limitation.



































We sincerely thank the reviewer for their insightful comments and questions, which have offered us a clear perspective on areas for improvement. Please see our responses below to clarify the main concerns. Also, if you feel that your original concerns have been resolved, we would appreciate it if you would update your evaluation to reflect this. Thank you!

## Clarification of Threat Model and High-Level Description

We are thankful for the reviewer's astute observation that our discussion has been primarily focused on the optimization perspective without a high-level exploration of our threat model. This approach is indeed a result of deep contemplation.

1. **Background and Classification of Attacks:**

/**
In the related work section, following previous studies, we categorize private textual data attacks into two main types: Malicious Attacks and Eavesdropping Attacks, the latter also referred to as Honest-but-Curious Server Attacks. However, we believe this classification oversimplifies the issue, missing many nuanced intermediary states. Traditional views hold that Malicious Attacks involve issuing malicious server states (parameters) or even altering model structures. Under such a definition, when an attack occurs, the federated learning protocol is compromised, as the generated gradient information is valueless for minimizing the loss. However, in our method, while we modify the model, we do not change the inherent purpose of the gradients and do not affect the original training of the model. From this perspective, our method does not align with a typical Malicious Attack. Our modifications are confined solely to the Pooler layer (including expanding the model's width and changing the activation function), and these modifications are relatively minor compared to those in Malicious Attacks.
**/

Following previous work, we categorized private data attacks as Malicious and Eavesdropping (or Honest-but-Curious Server) Attacks in our study, but this oversimplifies the issue. Traditional Malicious Attacks involve altering server states or model architecture, rendering gradient information useless. However, our method, which only modifies the Pooler layer of the model, doesn't affect the original training purpose, thus differing from typical Malicious Attacks.

2. **Wider Pooler Layer**

/*
While applying our method to Pooler Layers requires the model to be sufficiently wide (d_out >> d_in), it's important to note that this is a relative concept. If we only need to recover a small portion of the input X (n x d_in), say X' (n x d_in') where d_in' < d_in, then the required width of the model can be significantly reduced. This point is emphasized in Section 4, "Flexibility of Recovered Dimension." More crucially, as Large Language Models (LLMs) continue to grow in size, this prerequisite will become less critical. For instance, GPT-3 (175 billion parameters) has a dimension of 12288, which is more than sufficient for recovering d_in' = 50. For simplicity, we did not conduct experiments directly on GPT-3. Moreover, many previous works specifically target wider models for attacks, which is a common approach in privacy attacks. Our contribution lies in demonstrating that wider models amplify the risks of private textual data attacks in our setting.
*/

Applying our method to the Pooler layer, while requiring a wide setting (d_out >> d_in), depends on the recovery needs. For a small input portion (X' with d_in' < d_in), the required width reduces significantly, as detailed in Section 4: Flexibility of Recovered Dimension. With the growth of Large Language Models like GPT-3, which already exceeds the necessary dimensions (12288 for d_in' = 50), this width requirement becomes less vital. Moreover, our attack focus on wider models aligns with previous studies, revealing more risk in our settings.

3. **Activation Functions Change**
/*
Regarding activation functions, we have so far revealed the risks associated with functions like Silu, which have neither purely odd nor even higher-order derivatives. We believe this to be a significant contribution. For activation functions with higher-order derivatives that are purely odd or even, such as tanh or relu, we are still exploring their potential risks. The requirement of specific activation functions has been a common aspect in previous works, and we do not view this as a flaw. Instead, we see it as an intermediate finding on our path to achieving the final goal, one that is sufficiently noteworthy to draw the attention of the community.
*/

We've identified risks with activation functions like Silu, lacking purely even or odd higher-order derivatives. Our ongoing research includes assessing risks in functions with strictly odd or even derivatives, like tanh or relu. Many previous studies strengthen particular activation functions; we claim our discovery is a contribution instead of a drawback.

3. **Redefining 'Honest-but-Curious':**
Compared to Eavesdropping (Honest-but-Curious) attacks, our method does involve some modifications to the model. However, we suggest that 'honest' should not be narrowly defined as the server's absolute fidelity to clients. Instead, 'honest' should be understood as the server's adherence to its primary role of obtaining effective gradients and minimizing the model's loss function. By this definition, our approach falls under the Honest-but-Curious category.

4. **Clarifying Our Method's Positioning:**
In summary, our method cannot be classified as a Malicious or Eavesdropping Attack unless we redefine the Honest-but-Curious category. Our method, compared to Malicious Attacks, is more difficult to detect and does not violate the fundamental objective of federated learning. In contrast to Eavesdropping Attacks, our approach achieves more effective outcomes. Therefore, we mainly discuss our method from the perspective of optimization.

5. **Elaborating on the Threat Model:**
To address the reviewer's concerns, our final paper version will highlight our threat model as follows:
1) We do not fine-tune the model's word and positional embeddings. The gradients for these embeddings are non-zero for words in the client's training data, enabling easy recovery of client sequences.
2) The server operates under a redefined 'honest but curious' model, aiming to learn maximally from client data gradients without altering the learning protocol. Our work diverges from scenarios involving malicious servers forcing extensive data leaks; instead, we concentrate on an honest server setting, which presents a more challenging attack environment.

6. **Appendix for Enhanced Understanding:**
To aid the reviewer's understanding, we will include a table in the appendix of our revised manuscript. This table will delineate the differences between Malicious Attacks, Eavesdropping Attacks, and Honest-but-Curious Server attacks, with examples from previous work. And we also include the table to compare the difference between ours with LAMP and Wang's work.

## Novelty Concern 

We appreciate your insights regarding the novelty of our work and would like to clarify some aspects to better highlight the innovative elements of our research:

1. **Clarification on Contribution:**
    - In our paper, we did not claim that "identifying the issue of gradient-based attacks" was our contribution. This aspect was merely an analysis to delve into the underlying problem, serving as a basis for proposing our novel solution. Our innovation lies elsewhere, particularly in our approach to handling textual data privacy attacks using intermediate features.

2. **Distinction from Previous Work [1]:**
    - While we acknowledge the existence of previous work [1] utilizing intermediate features for attacks, it is important to emphasize that their scope was primarily within the realm of image data. As we have underscored in our manuscript, attacks on textual data present far greater challenges than those on image data, due to inherent differences in data representation and model architectures.
    - Significantly, our work is the first to apply the concept of using intermediate features in the context of private textual data attacks. Moreover, our methodology is fundamentally different from the example cited by you. We have developed a unique approach tailored to the specificities of textual data, which involves innovative techniques and considerations not addressed in the previously mentioned image-based work.
    - Given these distinctions, we believe that the novelty of our approach in applying intermediate features to private textual data attacks remains substantial and represents a significant advancement in this field.

## Question 3 Tone and Subjectivity
We are thankful for your observation regarding the subjective tone in our manuscript. We commit to making the necessary adjustments in the revised version. However, to clarify, **our use of the term "revolutionary" was not intended to describe our method (Contribution 4)**. Instead, it referred specifically to the novel metric we introduced for measuring information leakage of textual data. 

## Question 4 Optimization Objective Clarification
Thank you for highlighting the need for clarification regarding our optimization objective. Indeed, your observation brings an important aspect of our method to light. In our approach, we focus on recovering the directional component of the Pooler layer's input through decomposition techniques. However, accurately reconstructing the magnitude of this input remains a challenge. To address this limitation, we employ cosine similarity loss as our optimization criterion



## Question 2: Novelty Concern

Thank you for your comments on our work's novelty. We'd like to clarify a few points:

1. **Contribution Clarification:**
    - Our contribution isn't about identifying gradient-based attack issues, which was just an analysis foundation. Our innovation is in our unique approach to protecting textual data privacy using intermediate features.

2. **Differentiation from Prior Work [1]:**
    - We recognize similar use of intermediate features in previous studies [1] on image data. However, our work pioneers this concept for textual data attacks, facing unique challenges not seen in image data due to differences in data representation and model architectures.
    - Our methodology for textual data is distinctive and involves novel techniques, setting it apart from the image-based approaches previously discussed.
    - These differences underscore our method's novelty in applying intermediate features to textual data privacy, marking a significant contribution to the field.

## Question 3: Tone and Subjectivity
Thank you for pointing out the subjective tone. We will revise this. **The term "revolutionary" was specifically for our new metric on textual data information leakage, not our method (Contribution 4)**.

## Question 4: Optimization Objective
Appreciate your input on our optimization objective. We aim to recover the directional component of the Pooler layer's input using decomposition, acknowledging challenges in reconstructing its magnitude. Our solution employs cosine similarity loss to address this limitation.














==> src/rebuttal/rebuttal-2.tex <==
Thank you for your constructive feedback. Below are our responses to your main concerns. If these address your initial queries, we'd be grateful if you could revise your evaluation accordingly.

### Q1. Constraints of the Proposed Attack:
---

We recognize some limitations to a certain extent, but not entirely, as real-world attacks are often more extreme than this scenario. To provide further clarity, we compare our methodology from an attack perspective with prior research.

1. **Wide Pooler Layer Constraints:** The width of the Pooler Layer is adaptive to recovery needs. As we detailed in **Section 4: Flexibility of Recovered Dimension**, for smaller input portions (X' with d_r << d_in), the required width is significantly reduced. With advancements in Large Language Models like GPT-3, which already surpass necessary dimensions (12288 for d_r = 50), this width requirement becomes less critical. Furthermore, our focus on wide models aligns with previous studies (e.g., Geiping et al., 2020; Fowl et al., 2022), highlighting increased risks in our settings.

2. **Activation Functions Change:** We have identified risks related to using activation functions such as Selu, whose higher-order derivatives are neither odd nor even. Our ongoing research extends to activation functions with strictly odd or even derivatives, such as Tanh or Relu. While many previous studies have focused on specific activation functions (Zhu et al., 2019, Flow et al.2022), we view this discovery as a contribution, not a drawback.

3. **`Comparison with Previous Studies`:**
    - Previous works [e.g., Flow et al., 2022, 2023; Boenisch et al., 2023] have implemented attacks capable of handling very large batch sizes and long sequence text recovery. However, these methods, called Malicious Attacks, have critical flaws. Firstly, they violate the federated learning protocol, as the gradients returned by the client during an attack are meaningless. Secondly, they involve multi-layer modifications to model parameters or even insert new modules, which are far more aggressive than our modifications. In contrast, we only modify the Pooler Layer and consistently adhere to the federated learning protocol. Nevertheless, we recognize the value of these works in advancing privacy attack research.
    - Works like LAMP can extract private text information using only optimization-based techniques and prior knowledge without any model modifications. However, this is a self-imposed limitation. In reality, servers can undertake actions well beyond this scope. Although such actions may be more easily detectable, our method achieves less detectability while providing additional optimization signals, marking a significant innovation.

4. **`The Specificity of Attack Scenarios`:** Research in privacy attacks holds a unique importance in practice. This is because every discovery in this area, even with certain constraints, can cause tremendous destruction once happens. The attacker will try their best to satisfy the constraints because of the hidden massive profit. Therefore, the risks uncovered by these studies are often difficult to measure, making them crucial for understanding security vulnerabilities.

### Q2. Architecture of Evaluation Baselines
---

We are grateful for your observation regarding the architecture used in our baseline evaluations, and we would like to clarify this aspect to dispel any confusion.

In our comparative analysis, we maintained the original model structures of our baselines without altering their activation functions. This decision was driven by our goal to uncover potential private text attack methods, where the choice of activation function plays a crucial role. In our research, we discovered that activation functions with neither purely odd nor even higher-order derivatives, such as Selu or $x^3+x^2$, pose significant risks in our specific setting compared to more traditional functions like Relu/Tanh.

This discovery regarding the choice of activation functions is a part of our contribution. It highlights the vulnerabilities in real-world applications under our experimental conditions. Therefore, we do not consider the selection of activation functions as a distilled item for comparison with other methods. Instead, it is more pertinent to internal comparisons within our methodology. We have included a detailed discussion on this topic in the appendix.

### Q3. Clarification on Equations 5 & 6
---
    
We appreciate your request for further clarification regarding Equations 5 & 6, and we will provide more explanation in the appendix of our revised manuscript.

Regarding the uniqueness of $x_i$'s recovery, it largely depends on the correlation among different data points within the batch. In the appendix of our manuscript, we have a dedicated discussion section titled "Influence of Data Dependence", where we delve into how the cosine similarity between recovered features and actual features gradually decreases as batch size increases.


==> src/rebuttal/rebuttal-3.tex <==

Thank you for your constructive feedback. Below are our responses to your main concerns. If these address your initial queries, we'd be grateful if you could revise your evaluation accordingly.

### Q1: Clarification on the Novelty of Using Intermediate Features 
---

We sincerely appreciate your reference to the paper [HKHG+], which shares a similar intuition of shifting the focus from model input to intermediate features but in a completely different context.

1. **Different Context and Application:** Our work uniquely focuses on recovering textual data in LLMs within the context of federated learning (FL). The cited work [HKHG+] primarily examines the use of intermediate feature perturbation to enhance the transferability of adversarial inputs in the context of black-box adversarial attacks.

2. **Totally Different Methods**: Our method does not know the true intermediate feature, instead utilizing gradient information and tensor decomposition technique to estimate the feature. The reference [HKHG+] can easily calculate the intermediate features with the model and input.

To better respond to the reviewer's concern, we will present a discussion that delves into the underlying intuitions of both approaches, highlighting the differences and acknowledging the similarities where applicable.

### Q2: Risks in LLMs within FL
---

Thank you for inquiring about the privacy risks of textual data in LLMs within FL. To safeguard user privacy, users' textual data is typically stored on local edge devices. These devices compute gradient information and upload it to the central server. Ideally, the server doesn't access the original text, but studies have shown it's possible to reconstruct training text from gradient information and prior knowledge. We hope this clarifies the challenges in LLMs within FL.

### Q3 & Q5: Clarification on Notations
---

1. **[CLS] Token:** This special token, added at the start of each input sentence, is selected to represent the sentence for classification tasks.

2. **$\hat{x}$ and $\hat{y}$ in Equation 3:** These symbols are the optimization goal that represents the estimated input and label, respectively.

3. **B in Equation 2:** Refers to Batch Size.

4. **$\nabla^{3}g(w)$ and $x_{i}^{\otimes3}$:** $\nabla^{3}g(w)$ is the third derivative of $g(w)$, and $x_{i}^{\otimes3}$ signifies the tensor product of vector $x_{i}$ with itself three times.

### Q4: Clarification on security model
---

1. **Adversary in the Attack:** The server in FL is the adversary, operating under a redefined 'honest but curious' setting. It aims to learn as much text as possible from the gradients without altering the learning protocol. (`The honest here refers to the server always minimizing the training loss without other objectives`)

2. **Adversary's Ability:** The server can modify the Pooler layer of the model, allowing it first to recover the intermediate features (`No other prior knowledge`). However, the server does not finetune the word and positional embeddings (The gradients for these embeddings are non-zero for words in the client's training data, enabling easy recovery of client sequences).

3. **Action of Participants:** Clients compute the gradient and upload it to the server, which is benign.

4. **Security Implication:** This approach challenges traditional security models in FL. It's less detectable than Malicious Attacks and more invasive than typical Honest-but-Curious attacks, aiming to recover textual data from shared gradients. (`The honest here refers to the server not changing model architecture and parameters`)

5. **Attacking Goal:** The primary goal is to recover client sequences or information from the gradients `without deviating from the fundamental objectives of federated learning, like effective gradient aggregation and model loss minimization`.

### Q6: Theoretical Discussion.
---

We have addressed the reviewer's concern in the following sections:

1. **Bridging Experimental Findings with Theory:** In Section 5.3, "`Impact of Recovery Dimension`" and Appendix Section A.4, "`Influence of Data Dependence`" we have thoroughly discussed how our experimental findings correlate with the theoretical insights presented in (Wang et al., 2023).

2. **Discussion on Optimization Signals:** We have also explored the impact of different optimization signals in `the second and third paragraphs` of Section 5.3. Additionally, our ablation experiments in Section 5.4, “`Impact of Feature Match in Different Optimization Phases`”, further elaborate on how varying optimization signals influence attack performance.

### Q7：Comparison with Previous
---

Please refer to Section 5.3, "`Results and Analysis`", for a detailed explanation. The performance degradation observed in previous works when increasing the batch size is attributed to the gradient being averaged over more tokens and sentences. Our method introduces an additional supervisory signal that mitigates this issue.

==> src/rebuttal/rebuttal-4.tex <==
Thank you for your constructive feedback. Below are our responses to your main concerns. If these address your initial queries, we'd be grateful if you could revise your evaluation accordingly.

### Q1：Performance on Other Types of Tasks
---

Thank you for highlighting the importance of evaluating our proposed method's effectiveness in other natural language processing tasks, such as translation or generation tasks. We acknowledge that our approach might face greater challenges in these contexts. In such tasks, the loss generated by different tokens is typically summed or averaged before computing gradients, in contrast to classification tasks that usually produce a single loss.

1. **Acknowledging Shared Challenges in the Community:**： We recognize that these challenges are not unique to our method but are common obstacles faced across the community in privacy attack research. This issue underscores the complexity and variety of tasks in natural language processing and their implications for privacy attacks.

2. **Emphasizing the Practical Importance of Privacy Attack Research:**： We wish to emphasize that our primary goal is not to develop a universal privacy attack method but to highlight potential threats of LLMs within federated learning. It's essential to understand these vulnerabilities of the current protocol to prevent potential risks.

3. **Future Research Directions:**: Your concern aligns with our future research direction. We are motivated to explore how our attack methodology can be adapted or improved to address the unique challenges in tasks like translation and generation.

### Q2: Cost Analysis
---

We appreciate your attention to the cost implications of our method and would like to clarify two key aspects regarding this:

1. **Comparable Cost to Traditional Optimization-Based Techniques:**: Our method incurs almost the same computational cost as other traditional optimization-based techniques. This is primarily because the recovery of intermediate features in our approach involves a tensor decomposition technique, which is a one-time process. The computational effort for this part is negligible compared to the subsequent optimization steps. Moreover, during the optimization phase, our method only requires the additional computation of a cosine similarity loss, which also does not significantly increase the computational burden. Based on our assessments, our method does not add substantial extra computational overhead (less than 1.1 times the usual cost).

2. **Context of Attack Scenarios in Practice:**: It's important to consider the practical context of attack scenarios. Attackers often prioritize the effectiveness of the attack over the cost, implying that computational expense is not the primary concern in such research. This perspective is crucial in understanding the feasibility of privacy attacks, including ours, in real-world scenarios.

### Q3: Possible Countermeasures
---

We are grateful for your attention to both the attack methodologies and potential defense techniques in our study. We recognize the importance of defenses in the context of privacy attacks and appreciate this opportunity to discuss them.

1. **Effectiveness of Attack in Certain Settings:** Our research acknowledges that honest-but-curious type attacks on LLMs, especially when freezing the token and positional embeddings, tend to be effective primarily in settings with smaller batch sizes. While our method significantly improves the effectiveness of attacks for B > 1, we observe a notable decline in effectiveness when B > 8. This suggests that in federated learning scenarios with large batch sizes and a benign server, textual data privacy can still be reasonably safeguarded. (`The 'honest' here refers to the server's goal to recover client sequences or information from the gradients without deviating from the fundamental objectives of federated learning, like effective gradient aggregation and model loss minimization.`)

2. **Decision Against Including Defense Techniques:** Based on this observation, we chose not to focus on defense techniques within the scope of this paper. Our primary objective was to reveal the potential risk of privacy breaches in LLMs within federated learning settings, particularly those with moderate batch sizes.

Thank you again!

==> src/rebuttal/rebuttal-5.tex <==
Thank you for your constructive feedback. Below are our responses to your main concerns. If these address your initial queries, we'd be grateful if you could revise your evaluation accordingly.

### Q1: Contribution and Novelty of the Proposed Method
---

We appreciate your acknowledgment of our work's structure and ideas. However, it's crucial to emphasize that our approach is not a mere combination of existing methods; it includes several unique contributions:

1. **Theoretical vs. Practical Application:** Wang et al.'s work, while theoretically effective, encounters practical challenges due to various constraints that limit its effectiveness in real-world scenarios. In contrast, our approach adapts these theoretical insights to practical federated learning settings.

2. **Limitations in Wang et al.'s Work:** Wang et al.'s method is most effective in a two-layer neural network context. Extending it beyond this depth requires customizing model parameters, like identity matrices, which contradicts the definition of 'honest but curious' in federated learning. Our method maintains this 'honesty' by focusing on the top two layers of deep neural networks. (`The 'honest' here refers to the server's goal to recover client sequences or information from the gradients without deviating from the fundamental objectives of federated learning, like effective gradient aggregation and model loss minimization.`)

3. **Focus on Intermediate Feature Recovery:** Unlike Wang et al.'s work, which is limited to directly recovering model input, our method explores the potential of recovering intermediate features, adding a new dimension to attack strategies.

4. **Flexibility in Recovery Dimension:** Our approach offers more flexibility in optimizing recovery dimensions, as discussed in Section 4.2 "Flexibility of the Recovery Dimension." We can adaptively try different dimensions to meet specific needs, which is not the case in Wang et al.'s work.

5. **Innovative Weight Initialization Strategy:** We address the issue of gradients approaching zero due to weight randomization, as often happens in Wang et al.'s method. In Section 4.2 "Strategic Weight Initialization," we innovatively propose a coexistence of original and random weights, effectively overcoming this challenge.

6. **Addressing Data Point Order in Batches:** Wang et al.'s method struggles with determining the order of data points in the same batch. Our method, from an attacker's perspective, compares with the true features and adopts a greedy strategy based on the highest cosine similarity for one-to-one correspondence, effectively resolving the data point order issue.


### Q2 & Q3: Batch Size and Defense Methods
---

We recognize the importance of defenses in the context of privacy attacks and appreciate this opportunity to discuss them.

1. **Effectiveness of Attack in Certain Settings:** Our research acknowledges that honest-but-curious type attacks on LLMs, especially when freezing the token and positional embeddings, tend to be effective primarily in settings with smaller batch sizes. While our method significantly improves the effectiveness of attacks for B > 1, we observe a notable decline in effectiveness when B > 8. This suggests that in federated learning scenarios with large batch sizes and a benign server, textual data privacy can still be reasonably safeguarded.

2. **Decision Against Including Defense Techniques:** Based on this observation, we chose not to focus on defense techniques within the scope of this paper. Our primary objective was to reveal the potential risk of privacy breaches in LLMs within federated learning settings, particularly those with moderate batch sizes.

### Q4: Knowledge of Model Architecture
---

Thank you for raising the question about the attacker's knowledge of the model architecture; we clarify this as follows:

1. **Knowledge of Model Architecture in Security Settings:**
   - In the security model we've considered, whether the server setting is honest or malicious, the model's architecture is always known to the server. This knowledge is an inherent aspect of the federated learning setup, where the server orchestrates the learning process and, therefore, has access to the model architecture.

2. **Implications for Potential Hackers:**
   - Furthermore, even in scenarios where a hacker might steal model parameters, the limited variety of commonly used language models today often makes it possible to infer or guess the model architecture.

### 5：Definition of Private Information in Text
---

Thank you for your question. In your example, while 'delicious' isn't inherently sensitive, the key point is that attack methods don't distinguish between words like 'delicious' and genuinely sensitive information like personal health data. If our attack can recover something as benign as 'delicious,' it also has the potential to recover more sensitive information. Therefore, any potential data recovery is considered a privacy risk.

==> src/static/tables/table3.tex <==
\begin{table}[ht]
\small
\centering
\caption{Comparative analysis of different attack categories on textual data. Please note that we do not consider the attack methods that require fine-tuning the token and positional embeddings. (The term \textbf{\textit{honest}} signifies the server's intention to extract client sequences or information from gradients, while still adhering to the core principles of federated learning, such as efficient gradient aggregation and minimizing model loss).}
\begin{tabularx}{\textwidth}{l|c|c|C}
\hline
\hline
\textbf{Attack Category} & \textbf{Malicious} & \textbf{Eavesdropping} & \textbf{Honest-but-Curious (Ours)} \\
\hline
Degree of Model Modification & Heavy & None & Light \\
\hline
Model Modification & Multiple Layers & None & Single Layer \\
\hline
Insertion of New Module & Yes / None & None & None \\
\hline
Attack Constraint & Heavy & Light & Moderate \\
\hline
FL Protocol Broken & Yes & None & None \\
\hline
Attack Effectiveness & Strong & Weak & Moderate \\
\hline
& \citet{fowl2021robbing}  & \citet{balunovic2022lamp} &  \\
Studies & \cite{fowl2022decepticons} & \cite{zhu2019deep} & Ours \\
& \cite{boenisch2023curious} & \citet{deng2021tag} & \\
\hline
\end{tabularx}
\label{table:attack_categories}
\end{table}

